QED: Scalable Verification of Hardware Memory Consistency

Memory consistency model (MCM) issues in out-of-order-issue microprocessor-based shared-memory systems are notoriously non-intuitive and a source of hardware design bugs. Prior hardware verification work is limited to in-order-issue processors, to proving the correctness only of some test cases, or to bounded verification that does not scale in practice beyond 7 instructions across all threads. Because cache coherence (i.e., write serialization and atomicity) and pipeline front-end verification and testing are well-studied, we focus on the memory ordering in an out-of-order-issue processor's load-store queue and the coherence interface between the core and global coherence. We propose QED based on the key notion of observability that any hardware reordering matters only if a forbidden value is produced. We argue that one needs to consider (1) only directly-ordered instruction pairs -- transitively non-redundant pairs connected by an edge in the MCM-imposed partial order -- and not all in-flight instructions, and (2) only the ordering of external events from other cores (e.g.,invalidations) but not the events' originating cores, achieving verification scalability in both the numbers of in-flight memory instructions and of cores. Exhaustively considering all pairs of instruction types and all types of external events intervening between each pair, QED attempts to restore any reordered instructions to an MCM-complaint order without changing the execution values, where failure indicates an MCM violation. Each instruction pair's exploration results in a decision tree of simple, narrowly-defined predicates to be evaluated against the RTL. In our experiments, we automatically generate the decision trees for SC, TSO, and RISC-V WMO, and illustrate automatable verification by evaluating a substantial predicate against BOOMv3 implementation of RISC-V WMO, leaving full automation to future work.

==> figures/old-fig-tex/load_load_order.tex <==
\begin{tikzpicture}
[
ooonode/.style={rectangle, draw=black!60,dashed, fill=black!5, very thick, align=center, text width=20mm, minimum size=5mm},
instnode/.style={rectangle, draw=black!60, fill=black!5, very thick, align=center, text width=20mm, minimum size=5mm},
relnode/.style={rectangle, draw=black!0, fill=black!0, very thick, align=left, text width=18mm, minimum size=3mm},
capnode/.style={rectangle, draw=black!0, fill=black!0, very thick, align=center, minimum size=3mm},
]

\draw [black, ultra thick, ->] (5mm, 5mm) -- (5mm, -50mm);

\node [ooonode] (ldb1) [] {LD B};

\node [relnode] (rel1) [below right = 0mm and -5mm of ldb1] {\lo};

\node [instnode] (invb) [below right = 5mm and -15mm of ldb1] {INV B};

\node [relnode] (rel2) [below = 5mm of rel1] {\lm};

\node [instnode] (inva) [below = 5mm of invb] {INV A};

\node [relnode] (rel3) [below = 5mm of rel2] {\lo};


\node [instnode] (lda) [below left = 5mm and -15mm of inva] {LD A};

\node [relnode] (rel4) [below = 5mm of rel3] {\lp};

\node [instnode] (ldb2) [below = 5mm of lda] {LD B};

\draw [dashed, ultra thick, ->] (ldb2.west) to [out=120, in=240] (ldb1.west);

\node [capnode] (caption) [left = 0mm of inva] {out-of-order \\ reorder};

\end{tikzpicture}

==> figures/old-fig-tex/ooo_load_with_squash.tex <==
\begin{tikzpicture}
[
ooonode/.style={rectangle, draw=black!60,dashed, fill=black!5, very thick, align=center, text width=20mm, minimum size=5mm},
instnode/.style={rectangle, draw=black!60, fill=black!5, very thick, align=center, text width=20mm, minimum size=5mm},
relnode/.style={rectangle, draw=black!0, fill=black!0, very thick, align=left, text width=18mm, minimum size=3mm},
capnode/.style={rectangle, draw=black!0, fill=black!0, very thick, align=center, minimum size=3mm},
]

\draw [black, ultra thick, ->] (5mm, 5mm) -- (5mm, -40mm);

\node [ooonode] (ldb1) [] {LD A};

\node [relnode] (rel1) [below right = 0mm and -5mm of ldb1] {\lo};

\node [instnode] (invb) [below right = 5mm and -15mm of ldb1] {INV A};

\node [relnode] (rel2) [below = 5mm of rel1] {\lo};

% \node [instnode] (inva) [below = 5mm of invb] {INV A};

% \node [relnode] (rel3) [below = 5mm of rel2] {$<_m$};


\node [instnode] (instr) [below left = 5mm and -15mm of invb] {INSTR};

\node [relnode] (rel3) [below = 5mm of rel2] {\lp};

\node [instnode] (ldb2) [below = 5mm of instr] {LD A};

\draw [dashed, ultra thick, ->] (ldb2.west) to [out=120, in=240] (ldb1.west);

\node [capnode] (caption) [left = 0mm of invb] {out-of-order \\ reorder};

\node [relnode, text=red] (rel4) [below=5mm of rel3] {squash condition} ;

\draw [ultra thick, dashed, red] ($(ldb2.south)-(0mm,3mm)$) to [in=270, out=0] ($(invb.east)+(3mm,0mm)$) to [out=90, in=0] ($(ldb1.north)+(0mm,3mm)$) to [out=180, in=90] (caption.north) to [out=270, in=180] (rel2.west) to [out=0, in=90] ($(instr.east)+(3mm,0mm)$ ) to[out=270, in=0] (rel3.west) to [out=180, in=90] ($(ldb2.west)-(3mm,0mm)$) to [out=270, in=180] ($(ldb2.south)-(0mm,3mm)$);



\end{tikzpicture}

==> figures/old-fig-tex/store_load_order.tex <==
\begin{tikzpicture}
[
ooonode/.style={rectangle, draw=black!60,dashed, fill=black!5, very thick, align=center, text width=20mm, minimum size=5mm},
instnode/.style={rectangle, draw=black!60, fill=black!5, very thick, align=center, text width=20mm, minimum size=5mm},
relnode/.style={rectangle, draw=black!0, fill=black!0, very thick, align=left, text width=18mm, minimum size=3mm},
capnode/.style={rectangle, draw=black!0, fill=black!0, very thick, align=center, minimum size=3mm},
]

\draw [black, ultra thick, ->] (5mm, 5mm) -- (5mm, -50mm);

\node [ooonode] (ldb1) [] {LD B};

\node [relnode] (rel1) [below right = 0mm and -5mm of ldb1] {\lo};

\node [instnode] (invb) [below right = 5mm and -15mm of ldb1] {INV B};

\node [relnode] (rel2) [below = 5mm of rel1] {\lm};

\node [instnode] (era) [below = 5mm of invb] {EXT RD A};

\node [relnode] (rel3) [below = 5mm of rel2] {\lo};


\node [instnode] (sta) [below left = 5mm and -15mm of era] {ST A};

\node [relnode] (rel4) [below = 5mm of rel3] {\lp};

\node [instnode] (ldb2) [below = 5mm of sta] {LD B};

\draw [dashed, ultra thick, ->] (ldb2.west) to [out=120, in=240] (ldb1.west);

\node [capnode] (caption) [left = 0mm of era] {out-of-order \\ reorder};

\end{tikzpicture}
